Randomized Matrix-free Trace and Log-Determinant Estimators

We present randomized algorithms for estimating the trace and deter- minant of Hermitian positive semi-definite matrices. The algorithms are based on subspace iteration, and access the matrix only through matrix vector products. We analyse the error due to randomization, for starting guesses whose elements are Gaussian or Rademacher random variables. The analysis is cleanly separated into a structural (deterministic) part followed by a probabilistic part. Our absolute bounds for the expectation and concentration of the estimators are non-asymptotic and informative even for matrices of low dimension. For the trace estimators, we also present asymptotic bounds on the number of samples (columns of the starting guess) required to achieve a user-specified relative error. Numerical experiments illustrate the performance of the estimators and the tightness of the bounds on low-dimensional matrices; and on a challenging application in uncertainty quantification arising from Bayesian optimal experimental design.

==> def.tex <==
% This file includes the latex setting and the user defined macros.


% packages 
%\usepackage{caption}
\usepackage{booktabs}
\usepackage[mathscr]{euscript}
\usepackage{color,amsmath,amssymb,mathrsfs}
\usepackage{graphicx}
\usepackage{algorithmic,algorithm}
\usepackage{tikz,pgfplots}
\usepackage{upgreek}
\usepackage{showkeys,cite}
%\usepackage{MnSymbol}
\usepackage[normalem]{ulem}
\usepackage[pdfborder={0 0 0}, colorlinks=true, linkcolor=blue]{hyperref}

\usepackage{latexsym}

\hypersetup{pdfborder=0 0 0}

%\setlength{\parindent}{1.5em}
%\setlength{\parskip}{1.5pt}
%\usepackage{parskip}         % skips spaces and does not indent new paragraphs

%\usepackage{mathabx}
%\usepackage{hyperref}
%\usepackage[textsize=footnotesize,color=yellow]{todonotes}
%\usepackage[plainpages=false,colorlinks=true,citecolor=blue,filecolor=blue,linkcolor=blue,urlcolor=blue]{hyperref}
%\usepackage[colorlinks=true]{hyperref}
%\hypersetup{linkcolor=blue,urlcolor=blue,citecolor=red}
%\usepackage[pdfborder={0 0 0}, colorlinks=true, linkcolor=blue]{hyperref}
%\theoremstyle{plain}
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}



% hack to enable table of contents
\makeatletter
\def\addcontentsline#1#2#3{%
  \addtocontents{#1}{\protect\contentsline{#2}{#3}{\thepage}}}
\long\def\addtocontents#1#2{%
  \protected@write\@auxout
    {\let\label\@gobble \let\index\@gobble \let\glossary\@gobble}%
    {\string\@writefile{#1}{#2}}}

\setcounter{tocdepth}{3}
\newcommand\tableofcontents{%
    \section*{%\contentsname\\[1ex]\noindent
        \@mkboth{\noindent%
           \MakeUppercase\contentsname}{\MakeUppercase\contentsname}}%
    \@starttoc{toc}%
    }
\newcommand*\l@section[2]{%
  \ifnum \c@tocdepth >\z@
    \addpenalty\@secpenalty
    \addvspace{1.0em \@plus\p@}%
    \setlength\@tempdima{1.5em}%
    \begingroup
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      \leavevmode \bfseries
      \advance\leftskip\@tempdima
      \hskip -\leftskip
      #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\par
    \endgroup
  \fi}
\newcommand*\l@subsection{\@dottedtocline{2}{1.5em}{2.3em}}
\newcommand*\l@subsubsection{\@dottedtocline{3}{3.8em}{3.2em}}
\newcommand*\l@paragraph{\@dottedtocline{4}{7.0em}{4.1em}}
\newcommand*\l@subparagraph{\@dottedtocline{5}{10em}{5em}}
\makeatother
% --------------------- end hack


% -----------------------------------------------
% User defined macros
% -----------------------------------------------


\newcommand{\llangle}{\left\langle\kern-2.1\nulldelimiterspace\left\langle}
\newcommand{\rrangle}{\right\rangle\kern-2.1\nulldelimiterspace\right\rangle}

\newcommand{\COMSOL}{\textsc{Comsol}\ Multiphysics}
\newcommand{\MATLAB}{\textsc{Matlab}}

%\newcommand{\B}{\bar{B}}
%\newcommand{\Nm}{{N_m}}
%\renewcommand{\matrix}[1]{\ensuremath{\boldsymbol{#1}}}
%\renewcommand{\vec}[1] {\ensuremath{\boldsymbol{#1}}}
\renewcommand{\vec}[1]{{\mathchoice
                     {\mbox{\boldmath$\displaystyle{#1}$}}
                     {\mbox{\boldmath$\textstyle{#1}$}}
                     {\mbox{\boldmath$\scriptstyle{#1}$}}
                     {\mbox{\boldmath$\scriptscriptstyle{#1}$}}}}
\newcommand{\mat}[1]{\mathbf{{#1}}}
\newcommand{\psio}{\mathring{\Psi}}
\newcommand{\trace}{\mathsf{tr}}
\newcommand{\ave}[1]{\mathsf{E}\left\{ {#1} \right\}}
\newcommand{\var}[1]{\mathsf{Var}\left\{ {#1} \right\}}
\newcommand{\cov}[2]{\mathsf{Cov}\left\{ {#1},{#2} \right\}}
\newcommand{\normf}[1]{\left\| {#1} \right\|_F}
\newcommand{\norm}[1]{\left\| {#1} \right\|}
\renewcommand{\span}{\mathsf{span}}
\renewcommand{\rank}{\mathsf{Rank}}
\renewcommand{\diag}{\mathsf{diag}}
\newcommand{\prob}{\mathsf{Prob}}
\newcommand{\uobs}{\vec{u}^{\mathsf{obs}}}
\newcommand{\uobsi}{u^{\mathsf{obs}}}
\newcommand{\vphi}{\varphi}
\newcommand{\eps}{\varepsilon}
\newcommand{\W}{\bar{W}}
\newcommand{\Nt}{{N_t}}
\newcommand{\Ns}{{N_s}}
\newcommand{\Nm}{{n}}
\newcommand{\Ntau}{{N_{\tau}}}
\newcommand{\Ntr}{{N_{{\mathsf{tr}}}}}
\newcommand{\ind}{\mathop{\chi}}
\newcommand{\uu}{\vec{\bar{u}}}
\newcommand{\dd}{\vec{\bar{d}}}
\newcommand{\BB}{\matrix{B}}
\newcommand{\WW}{\matrix{{W}}}
\renewcommand{\Xi}{X^{-1}}
\newcommand{\ip}[2]{\left\langle{#1}, {#2}\right\rangle}
\newcommand{\mip}[2]{\left\langle{#1}, {#2}\right\rangle_{\!\scriptscriptstyle{\text{M}}}}
%\newcommand{\mip}[2]{\llangle{#1}, {#2}\rrangle}
\newcommand{\design}[2]{\left\{ \begin{array}{c} {#1}\\{#2} \end{array}\right\}}
\newcommand{\note}[1]{{\textcolor{blue}{#1\,}}}
\newcommand{\alennote}[1]{\noindent\emph{\textcolor{red}{Alen: #1\,}}}
\newcommand{\gsnote}[1]{\noindent\emph{\textcolor{green}{GS: #1\,}}}
\newcommand{\nnote}[1]{\noindent\emph{\textcolor{orange}{N: #1\,}}}
\newcommand{\dbeta}{\ensuremath{\vec{\beta}}}
\newcommand{\vv}{\ensuremath{\vec{v}}}
%\newcommand{\ff}{\ensuremath{\vec{f}}}
\newcommand{\gbf}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\edot}{\dot{\ten{\varepsilon}}}
\newcommand{\secinve}{\edot_\mathrm{I\!\!\:I}}
\renewcommand{\matrix}[1]{\mathbf{#1}}
\renewcommand{\H}{\ensuremath{\matrix{H}}}
\newcommand{\M}{{\ensuremath{\matrix{M}}}}
\newcommand{\Minv}{\ensuremath{\matrix{M}^{-1}}}
%\newcommand{\W}{{\ensuremath{\matrix{W}}}}
\newcommand{\IA}{{\ensuremath{\mathscr{I}_A}}}
\newcommand{\K}{{\ensuremath{\matrix{K}}}}
\newcommand{\I}{{\ensuremath{\matrix{I}}}}
\newcommand{\A}{{\ensuremath{\matrix{A}}}}
\newcommand{\B}{{\ensuremath{\matrix{B}}}}
\newcommand{\V}{{\ensuremath{\matrix{V}}}}
\newcommand{\Cb}{{\ensuremath{\matrix{C}}}}
\renewcommand{\L}{{\ensuremath{\matrix{L}}}}
\newcommand{\F}{{\ensuremath{\matrix{F}}}}
\newcommand{\iF}{{\ensuremath{\vec{F}}}}
\newcommand{\g}{\ensuremath{\boldsymbol{g}}}
\newcommand{\h}{\ensuremath{\boldsymbol{h}}}
\newcommand{\nn}{\ensuremath{\boldsymbol{n}}}
\renewcommand{\v}{{\vv}}
\renewcommand{\u}{\ensuremath{\boldsymbol{u}}}
\newcommand{\w}{\ensuremath{\boldsymbol{w}}}
\newcommand{\FT}{\matrix{\tilde{F}}}
\newcommand{\HT}{\matrix{\tilde{H}}_{\text{misfit}}}
\newcommand{\HTr}{\matrix{\tilde{H}}_{\text{misfit},r}}
\newcommand{\HMb}{\matrix{\bar{H}}_{\text{misfit}}}
\newcommand{\HM}{\matrix{H}_{\text{misfit}}}
\newcommand{\HTinf}{\tilde{H}_{\text{misfit}}}
%\newcommand{\diag}{\text{diag}}
\newcommand{\blkdiag}{\mathsf{blkdiag}}


%\newcommand{\obs}{\vec{y}}  % Finite dimensional observations
\newcommand{\obs}{\vec{d}}  % Finite dimensional observations
\newcommand{\ipar}{m}
\newcommand{\dpar}{\vec{m}}
\newcommand{\iparmap}{\ipar_\text{\tiny{MAP}}}
\newcommand{\iparpost}{\ipar_\text{post}}
\newcommand{\dparmap}{\dpar_\text{MAP}}
\newcommand{\dparpost}{\dpar_\text{post}}
\newcommand{\Nel} {\ensuremath{{n_\text{el}}}}
\newcommand{\De} {\ensuremath{{\mathsf{D}^e}}}

% spatial point
\newcommand{\xx}{\ensuremath{\boldsymbol x}}
\newcommand{\rr}{\ensuremath{\boldsymbol r}}
\newcommand{\e}{\ensuremath{\boldsymbol e}}
\newcommand{\x}{\xx}
\newcommand{\y}{\ensuremath{\boldsymbol y}}
\newcommand{\z}{\ensuremath{\boldsymbol z}}
\renewcommand{\r}{\ensuremath{\boldsymbol r}}
\newcommand{\s}{\ensuremath{\boldsymbol s}}

\newcommand{\pp}{\ensuremath{\boldsymbol p}}
\newcommand{\qq}{\ensuremath{\boldsymbol q}}
\newcommand{\mm}{\ensuremath{\boldsymbol m}}

\newcommand{\mcempty}{\multicolumn{1}{c}{}}
\newcommand{\mcone}[1]{\multicolumn{1}{|c}{#1}}
\newcommand{\mctwo}[1]{\multicolumn{2}{|c}{#1}}

%\newtheorem{theorem}{Theorem}

\newcommand{\seclab}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figlab}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\theolab}[1]{\label{theo:#1}}
\newcommand{\theoref}[1]{\ref{theo:#1}}
\newcommand{\eqnlab}[1]{\label{eq:#1}}
\newcommand{\eqnref}[1]{\eqref{eq:#1}}
\newcommand{\lemlab}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{\ref{lem:#1}}

\newcommand{\titlefirstnote}{\raisebox{9pt}{$\ast$}}

\definecolor{pacificorange}{cmyk}{.15,.45,1,0} %approved Pacific colors 2010
\definecolor{pacificgray}{cmyk}{0,.15,.35,.60}
\definecolor{pacificlgray}{cmyk}{0,0,.2,.4}
\definecolor{pacificcream}{cmyk}{.05,.05,.15,0}
\definecolor{deepyellow}{cmyk}{0,.17,.80,0}
\definecolor{lightblue}{cmyk}{.49,.01,0,0}
\definecolor{lightbrown}{cmyk}{.09,.15,.34,0}
\definecolor{deepviolet}{cmyk}{.79,1,0,.15}
\definecolor{deeporange}{cmyk}{0,.59,1,.18}
\definecolor{dustyred}{cmyk}{0,.7,.45,.4}
\definecolor{grassgreen}{RGB}{92,135,39}
\definecolor{pacificblue}{RGB}{59,110,143}
\definecolor{pacificgreen}{cmyk}{.15,0,.45,.30}
\definecolor{deepblue}{cmyk}{1,.57,0,.2}
\definecolor{turquoise}{cmyk}{.43,0,.24,0}
\definecolor{green}{rgb}{0,0.65,0}

\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\ten}[1] {\ensuremath{\boldsymbol{#1}}}
\newcommand{\tenfour}[1]{\mathsf{#1}}
\newcommand{\tcb}[1]{\textcolor{blue}{{#1}}}
\newcommand{\tcm}[1]{\textcolor{grassgreen}{{#1}}}
\newcommand{\tco}[1]{\textcolor{deepviolet}{{#1}}}
\newcommand{\tcg}[1]{\textcolor{deeporange}{{#1}}}
\newcommand{\CC}{\ensuremath{c}}
\newcommand{\tCC}{\ensuremath{\tilde{c}}}

%\newcommand{\equaldef}{\stackrel{\mathrm{def}}{=}}
\newcommand{\equaldef}{{:=}}
\newcommand{\mb}[1]{\mathbf{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\nor}[1]{\left\| #1 \right\|}
\newcommand{\snor}[1]{\left| #1 \right|}
\renewcommand{\v}{\mb{v}}
\renewcommand{\u}{p}
\newcommand{\yobs}{\obs^{\text{obs}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\half} {\ensuremath{\frac{1}{2}}}
%\newcommand{\D}{\Omega}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Acal}{\mc{A}}
\newcommand{\borel}{\mathfrak{B}}
\newcommand{\hilb}{\mathscr{H}}
\newcommand{\Hcal}{\mc{H}}
\newcommand{\G}{\mathscr{L}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\X}{X}
\newcommand{\Y}{Y}
\newcommand{\C}{\mc{C}}
\newcommand{\Grad} {\ensuremath{\nabla}}
\newcommand{\DD}[2] {\ensuremath{\frac{d {#1}}{d {#2}}}}
\newcommand{\Ex}{\mathbb{E}}
\newcommand{\E}{E}
\newcommand{\LRp}[1]{\left( #1 \right)}
\newcommand{\LRs}[1]{\left[ #1 \right]}
\newcommand{\LRa}[1]{\left< #1 \right>}
\newcommand{\LRc}[1]{\left\{ #1 \right\}}
\newcommand{\GM}[2]{\mc{N}\left( #1, #2 \right)}
\newcommand{\del}{\partial}
\newcommand{\delj}[1]{\frac{\partial{#1}}{\partial {w_j}}}
\newcommand{\map}{\params_{\rm{MAP}}}
\newcommand{\dt}{\mathrm{d}t}
\newcommand{\dz}{\mathrm{d}z}
\newcommand{\proposal}{\bs y}
\newcommand{\params}{\bs m}
\newcommand{\paramcomponent}[1]{m_{#1}}
%\newcommand{\noise}{\bs e}
\newcommand{\obsop}{\mathcal{B}}
\newcommand{\observables}{\bs d}
\newcommand{\data}  { \observables_{\rm{obs}} }
\newcommand{\datacomponent}[1]{ \observables_{\rm{obs}}^{#1} }
\newcommand{\noise}  { \pi_{\rm{\scriptscriptstyle{noise}}}   }
\newcommand{\prior}  { \pi_{\rm{\scriptscriptstyle{prior}}}   }
\newcommand{\like}{ \pi_{\rm{\scriptscriptstyle{like}}} }
\newcommand{\post}{ \Pi_{\rm{post}} }
\newcommand{\postm}{\mu_{\rm{post}}}
\newcommand{\priorm}{\mu_0}
\newcommand{\ncov} {\bs \Gamma_{\rm{noise}} }
\newcommand{\nsigma} {\sigma_{\rm{noise}} }
\newcommand{\prcov} {\bs \Gamma_{\rm{prior}}    }
\newcommand{\postcov} {\bs \Gamma_{\rm{post}}    }
\newcommand{\prcovcomponent}[1] { \Gamma_{\rm{prior}}^{#1} }
\newcommand{\Lpr}     {\bs L}
\newcommand{\prmean}{ \bar{\params}_{\rm{prior}} }
\newcommand{\prmeancomponent}[1]{ \bar{\params}_{\rm{prior}}^{#1} }
\newcommand{\model}{\bs f(\params) }
\newcommand{\modelcomponent}[1]{ f_{#1}(\params)}
\newcommand{\misfit}{ \model - \data }
\newcommand{\ricker}{F^{\textrm{ricker}}(t)}
\newcommand{\cost}{J(\params)}
\newcommand{\costapprox}{\tilde J(\params)}
\newcommand{\obsmatrix}{\bs W}
\newcommand{\regmatrix}{\bs R}
\newcommand{\Hpost}  { \bs H }
\newcommand{\Hmisfit}{ \bs H_{\rm{misfit}} }
\newcommand{\Hmod}   {\tilde{\bs H}}
\newcommand{\gradpost}   {\bs g}
\newcommand{\vectorzero} {\bs 0}
\newcommand{\Vr} {\matrix{V}_r}
\newcommand{\Lr} {\matrix{\Lambda}_r}
\newcommand{\Dr} {\matrix{D}_r}
\newcommand{\Ir} {\matrix{I}_r}
\newcommand{\ML}{\M_l}
\newcommand{\Mt}{\tilde{\M}}
%\newcommand{\Mt}{\stackrel{\sim}{\smash{\M}\rule{0pt}{1.1ex}}}
\newcommand{\iFF}{\mathcal{F}}
\newcommand{\ff}{\mathcal{F}}     % I changed this to use the same symbol for parameter-to-observable map
\newcommand{\FF}{\matrix{F}}
\newcommand{\isol}{\mathcal{S}}
\newcommand{\sol}{\matrix{S}}
\newcommand{\dw}{\frac{\partial}{\partial w_i}}

% Macros for three different forms of adjoint operator
\newcommand{\adjMacroMM}[1]{{#1}^*}
%\newcommand{\adjMacroME}[1]{{#1}^\natural}
\newcommand{\adjMacroME}[1]{{#1}^*}
%\newcommand{\adjMacroEM}[1]{{#1}^\diamond}
\newcommand{\adjMacroEM}[1]{{#1}^*}
\newcommand{\adjMacroEMINV}[1]{{#1}^{-\diamond}}
\newcommand{\Aadj}{\adjMacroMM{\A}}
\newcommand{\Badj}{\adjMacroMM{\B}}
\newcommand{\iFFadj}{\adjMacroME{\iFF}}
\newcommand{\iFadj}{\adjMacroME{\iF}}
\newcommand{\Fadj}{\adjMacroME{\F}}
\newcommand{\Vadj}{\adjMacroEM{\V}}
\newcommand{\Ladj}{\adjMacroEM{\L}}

\newcommand{\wopt}{\vec{w}_{\text{opt}}}


\def\bfG{\mbox{\boldmath$G$}}
\setlength{\emergencystretch}{20pt}

\newcommand{\SNR}{\ensuremath{\text{SNR}}}



==> rademacher.tex <==
\begin{proof} The proof proceeds in three steps.  
\paragraph{1. Bound for ${\mom_2}$} The proof uses the matrix Rademacher series inequality~\ref{t_mat_ser}. Define the variance
\[ \sigma^2 \equiv \max\{\normtwo{\expect{\mom_2\mom_2^*}},\normtwo{\expect{\mom_2^*\mom_2}} \}. \]
Write $\mom_2\mom_2^*$ as a sum of outer products of the columns $\omega_i$ of $\mom_2$
\[\mom_2\mom_2^* = \sum_{i=1}^\ell \vomega_i\vomega_i^T \qquad \expect{\mom_2\mom_2^*} = \ell I_{n-k}.  \] 
%A calculation similar to~\cite[Section 4.4.2]{opp2015introduction} shows that $\sigma^2 = \nu_1$. 
By a similar calculation  $\expect{\mom_2^*\mom_2} =  (n-k)\mi_{k+p}$. As a result, $\sigma^2 = \nu(\mom_2)$. Write $\mom_2 = \sum_{i = 1}^{n-k} \sum_{j=1}^{k+p}\omega_{ij} \me_{ij}$, where $\omega_{ij}$ is the $(i,j)$-th entry of $\mom_2$ and $\me_{ij}$ has zero entries except for unity in the $(i,j)$-th entry. Since $\mom_2$ satisfies the conditions of~\ref{t_mat_ser} we have 
\begin{equation}\label{omega2_rad}
\prob{\normtwo{\mom_2} \geq u } \leq \> (n-k +\ell)\exp\left(-\frac{u^2}{2\nu(\mom_2)} \right). 
\end{equation}•


\paragraph{2. Bound for $\mom_1^\dagger$} The proof uses the matrix Chernoff concentration inequality. Let $\omega_i \in \mathbb{R}^{k\times 1}$ be the $i$-th column of $\mom_1$. Define $ \my \equiv \mom_1^*\mom_1$ and 
\[ \expect{\my} = \expect{\mom_1\mom_1^*} = \sum_{i=1}^\ell \expect{\vomega_i\vomega_i^T} = \ell I_k. \]
Furthermore, define $\mu_\text{min} (\my) \equiv \lambda_\text{min} (\expect{\my})$ and $\mu_\text{max} (\my) \equiv \lambda_\text{max} (\expect{\my})$. Clearly $\mu_\text{min} = \mu_\text{max} = \ell $. Observe that $\my$ can be written as a finite sum of rank-1 matrices, each with maximum eigenvalue $\vomega_i^T\vomega_i \leq k$. $\mom_1$ satisfies the conditions of the matrix Chernoff theorem~\cite{TroppBook}. Therefore, by~\ref{t_mat_chern}, for $\epsilon \in [0,1)$ we have 
\[ \prob{\lambda_\text{min}(\mom_1\mom_1^*)  \leq (1-\epsilon) \ell } \leq k \left[\frac{e^{-\epsilon}}{(1-\epsilon)^{1-\epsilon}}\right]^\frac{\ell}{k}.  \]
Define $g(x) = e^x/(1+x)^{(1+x)}$. Next observe that $-\log g(-\epsilon)$ has the Taylor series expansion in the region $0 < \epsilon < 1$ 
\[ -\log g(-\epsilon) = \epsilon + (1-\epsilon)\log(1-\epsilon)  = \frac{\epsilon^2}{2} +  \frac{\epsilon^3}{6} +  \frac{\epsilon^4}{12} + \dots   \]
so that $-\log g(-\epsilon) \leq \epsilon^2/2$ for $0 < \epsilon < 1$ or $g(-\epsilon) \leq e^{-\epsilon^2/2}$. This gives us
\[  \prob{\normtwo{\mom_1^\dagger}^2  \geq  \frac{1}{ (1-\epsilon) \ell } }\>  \leq \> k  \exp\left(-\frac{\epsilon^2\ell}{2k}\right) . \]


\paragraph{3. Combining bounds} Define the event 
\[E_l = \left\{  \normtwo{\mom_1^\dagger}^2 \leq  \frac{1}{\ell (1-\epsilon)} \right\}, \]
and therefore, the complementary event $E_l^c$ satisfies $\prob{E_u^c} \leq k \exp\left(-\frac{\epsilon^2\ell}{2k}\right)  $. Conditioning the bound for $\mom_2$ on the event $E_c$, 
\[\prob{\normtwo{\mom_2} \geq u \left| E_\ell \right. } \leq \> (n-k + \ell)\exp\left(-\frac{u^2}{2\nu(\mom_2)} \right). \] 
Removing the conditioning from event $E_\ell$, we have 
\[ \prob{\normtwo{\mom_2}^2\normtwo{\mom_1^\dagger}^2 \geq \frac{u}{(1-\epsilon)\ell} } \leq  (n-k+\ell)\exp\left(-\frac{u}{2\nu(\mom_2)}\right)  + k\exp\left(-\frac{\epsilon^2\ell}{2k}\right).   \]  
For this event to happen with probability $\delta$,
\[\frac{\delta}{2} = (n-k+\ell )\exp\left(-\frac{u}{2\nu}\right) \qquad  \frac{\delta}{2} = k \exp\left(-\frac{\epsilon^2\ell}{2k}\right) . \]
Solving for $u$ gives us  $u = 2\nu \log\frac{2(n-k+\ell)}{\delta}$ and the solution for $\ell$ is provided in the statement of the Theorem. The result follows by plugging in the expression for $u$.   

\end{proof}


